Enhancing Multivariate Time Series Forecasting with Mutual Information-driven Cross-Variable and Temporal Modeling

Recent advancements have underscored the impact of deep learning techniques on multivariate time series forecasting (MTSF). Generally, these techniques are bifurcated into two categories: Channel-independence and Channel-mixing approaches. Although Channel-independence methods typically yield better results, Channel-mixing could theoretically offer improvements by leveraging inter-variable correlations. Nonetheless, we argue that the integration of uncorrelated information in channel-mixing methods could curtail the potential enhancement in MTSF model performance. To substantiate this claim, we introduce the Cross-variable Decorrelation Aware feature Modeling (CDAM) for Channel-mixing approaches, aiming to refine Channel-mixing by minimizing redundant information between channels while enhancing relevant mutual information. Furthermore, we introduce the Temporal correlation Aware Modeling (TAM) to exploit temporal correlations, a step beyond conventional single-step forecasting methods. This strategy maximizes the mutual information between adjacent sub-sequences of both the forecasted and target series. Combining CDAM and TAM, our novel framework significantly surpasses existing models, including those previously considered state-of-the-art, in comprehensive tests.

==> icml2024/section/approach.tex <==
\section{Method}
In multivariate time series forecasting, one aims to predict the future value of time series $y_{t}=s_{t+T+1:t+T+P} \in \mathbb{R}^{P \times C}$ given the history $x_{t}=s_{t:t+T} \in \mathbb{R}^{T \times C}$, where $T$ and $P$ refer the number of time steps in the past and future. $C \geq 1$ refers the number of variables. Given time series $s$, we divide it into history set $X=\{ x_{1},...,x_{N} \}$ and future set $Y=\{ y_{1},...,y_{N} \}$, where $N$ is the number of samples. As depicted in Figure~\ref{fig:intro_example} (a), deep learning methods first extract latent representation $Z^{i}$ from $X$ (Channel-mixing) , or $X^{i}$ (Channel-independence) , and subsequently generate target series $Y^{i}$ from $Z^{i}$.
A natural assumption is that these $C$ series are associated which helps to improve the forecasting accuracy. To leverage the cross-variable dependencies while eliminating superfluous information, in Section~\ref{approach:CAM}, we propose the \textbf{C}ross-Variable Decorrelation \textbf{A}ware Feature \textbf{M}odeling (\mf) to extract cross-variable dependencies. Additionally, in section~\ref{approach:TAM}, we introduce \textbf{T}emporal \textbf{A}ware \textbf{M}odeling (\ms) that explicitly models the correlation of predicted series and allows to generate more accurate predictions compared to the single-step forecaster.


%As aforementioned, we have highlighted the difficulties of multivariate time series forecasting: eliminate irrelevant cross-variable information and enhance temporal relationships for future series. To tackle these two challenges, we introduce \framework \xspace based on Mutual Information theory which consists of \mf \xspace and \ms.
\subsection{Cross-Variable Decorrelation Aware Feature Modeling}
\label{approach:CAM}
% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.42]{figure/method_1.pdf}
% \caption{(a) The framework of Channel-Independent model and Channel-Dependent model. The Channel-Dependent model tends to maximize the mutual information between historical series $X$ and latent representation $Z^{i}$ the mutual information between $Z^{i}$ and $i$-th future series $Y^{i}$. The Channel-Independent model maximizes the mutual information between i-th historical series and $Z^{i}$ and ignores the mutual information between $Z^{i}$ and other channels; (b) Traffic flow of 5 \textcolor{red}{five} adjacent detectors in \textcolor{red}{the} PEMS08 dataset; and (c) Prediction results of PatchTST using Single Channel feature and Multi-Channel feature respectively (we use two linear layers with Tanh activation to extract Multi-Channel feature)}
% \label{fig:framework}
% \end{figure}
 %In order to enhance the relationship between the latent representation $Z^{i}$ and the $i$-th historical series meanwhile eliminating the irrelevant cross-variable information, inspired by Information Bottleneck theory~\cite{tishby2000information}, we have the objective:
Recent studies~\citep {nie2022time,zeng2022transformers,zhou2021informer,zhang2023crossformer} have demonstrated that  Channel-independence is more effective in achieving high-level performance than Channel-mixing. 
%However, multivariate time series contain correlations among variables. Channel-mixing aims to take advantage of these cross-variable dependencies to predict future series. 
However, it is important to note that multivariate time series inherently contain correlations among variables. Channel-mixing aims to leverage these cross-variable dependencies for predicting future series, but it often fails to improve the performance of MTSF. One possible reason for this is that Channel-mixing introduces superfluous information.
%In fact, it fails to improve the performance of MTSF.  This may be because Channel-mixing introduces that superfluous information.
To verify this, we introduce \mf \xspace to extract cross-variable information while eliminating superfluous information. Specifically, drawing inspiration from information bottlenecks, \mf \xspace maximizes the joint mutual information among the latent representation $Z^{i}$, its univariate input $X^{i}$ and the corresponding univariate target series $Y^{i}$. Simultaneously, it minimizes the mutual information between latent representation $Z^{i}$ of one single univariate time series and other multivariate series input $X^{o}$. This leads us to formulate the following objective:

 \begin{equation}
    \max \,\, I(Y^{i},X^{i};Z^{i})  \,\, s.t. \,\, I(X^{o};Z^{i})\leq { I_{c}},
\end{equation}
%\begin{equation}
%    \max \,\, I(Y^{i};Z^{i})  \,\, s.t. \,\, I(X^{o};Z^{i}|X^{i})+I(Z^{i};X^{i}) \leq I_{c}  .
%\end{equation}
% {where $I_{c}$ is the information constraint}, $X$ is the set of multivariate historical series, $X^{i}$ is the historical series of $i$-th variable , $X^{o}$ is the other multivariate series, $Z^{i}\in \mathbb{R}^{d}$ is the representation of %$X_i$ 
% {$X^{i}$} via mixing  $X^{o}$ and used to predict the $i$-th future series $Y^{i}$.
%\wenlj{\sout{For Channel-mixing model, we directly utilize its latent representation $Z^{i}$; For Channel-Independence model, since it only extracts univaraite representation, we additionally utilize MLP for Channel-mixing. }} 

where $I(Y^{i},X^{i};Z^{i})$ represents the joint mutual information between the target series $Y^{i}$, the univariate input $X^{i}$, and the latent representation $Z^{i}$. Additionally, $I(X^{o};Z^{i})$ represents the mutual information between the latent representation $Z^{i}$ and the other multivariate input series $X^{o}$. The constraint $I(X^{o};Z^{i})\leq I_{c}$ ensures that the mutual information between $X^{o}$ and $Z^{i}$ is limited to a predefined threshold $I_{c}$.

With the introduction of a Lagrange multiplier $\beta$, we can maximize the objective function for the i-th channel as follows:
% we can maximize the objective function for {$i$-th channel}:
% \begin{equation}
% \begin{aligned}
%     \mathcal{R}_{IB}^{i}&= I(Y^{i};Z^{i}|X^{i}) -\beta I(X;Z^{i}) + I(X^{i};Z^{i}) \\
% \end{aligned}
% \end{equation}
\begin{equation}
\label{ib}
    \begin{aligned}
\mathcal{R}_{IB}^{i}&=I(Y^{i},X^{i};Z^{i})- \beta I(X^{o};Z^{i}) \\
        &=I(Y^{i};Z^{i}|X^{i})+ I(X^{i};Z^{i}) -\beta I(X^{o};Z^{i}),
        \end{aligned}
\end{equation}
where $\beta \geq 0$ controls the tradeoff between $I(Y^{i};Z^{i}|X^{i})$, $I(X^{i};Z^{i})$ and $I(X^{o};Z^{i})$, the larger $\beta$ corresponds to lower mutual information between $X^{o}$ and $Z^{i}$,
% and also means that $Z^{i}$ needs to retain the important information in $X^{o}$ and eliminate the irrelevant information to ensure $Y^{i}$ can be accurately predicted. 
indicating that $Z^{i}$ needs to retain important information from $X^{o}$ while eliminating irrelevant information to ensure accurate prediction of $Y^{i}$.
% However, the Mutual Information $I(X^{i},Y;Z^{i})$ and $I(X^{o};Z^{i})$ are intractable, we now provide the variational lower bound and upper bound for $I(X^{i},Y^{i};Z^{i})$ and $I(X^{o};Z^{i})$, respectively.
However, the computation of mutual information $I(X^{i},Y^{i};Z^{i})$ and $I(X^{o};Z^{i})$ is intractable. Therefore, we provide variational lower bounds and upper bounds for $I(X^{i},Y^{i};Z^{i})$ and $I(X^{o};Z^{i})$, respectively.

\textbf{Lower bound for} $I(X^{i},Y^{i};Z^{i})$. 
%The Mutual Information between the $i$-th historical series $X^{i}$, $i$-th target series $Y^{i}$ and the latent representation $Z^{i}$ is defined as (More details are shown in Appendix~\ref{sec:a.2})
The joint mutual information between latent representation $Z^{i}$, i-th historical series $X^{i}$, and i-th target series $Y^{i}$ is defined as (More details are shown in Appendix~\ref{sec:a2.1}):
\begin{equation}
    \begin{aligned}
        I(X^{i},Y^{i};Z^{i})&=I(Z^{i};X^{i}) +I(Z^{i};Y^{i}|X^{i})  \\
        &=\E_{p(z^{i},y^{i},x^{i})} \left[ \log p(y^{i}|x^{i},z^{i})\right] \\
        &+\E_{p(z^{i},x^{i})} \left [ \log p(x^{i}|z^{i}) \right] + H(Y^{i},X^{i}),  \\
    \end{aligned}
\end{equation}
where the joint entropy $H(Y^{i},X^{i})=-\int p(y^{i},x^{i})dx^{i}dy^{i}$ is only related to the dataset and cannot be optimized, so can be ignored. 
Therefore, the MI can be simplified as: 
%is independent of the optimization procedure and so can be ignored. Therefore, the MI can be simplified as: 
\begin{equation}
\begin{aligned}
    I(X^{i},Y^{i};Z^{i}) &=\E_{p(z^{i},y^{i},x^{i})} \left[ \log p(y^{i}|x^{i},z^{i})\right] \\
    &+\E_{p(z^{i},x^{i})} \left [ \log p(x^{i}|z^{i}) \right]+\text{constant}.
\end{aligned}
\end{equation}
Since $p(y^{i}|x^{i},z^{i})$ and $p(x^{i}|z^{i})$ are intractable, we introduce $p_{\theta}(y^{i}|z^{i},x^{i})$ and $p_{\theta}(x^{i}|z^{i})$ to be the variational approximation to $p(y^{i}|x^{i},z^{i})$ and $p(x^{i}|z^{i})$, respectively. Thus the variational lower bound can be expressed as (More details are shown in Appendix~\ref{sec:a2.2}):
\begin{align}
    I(X^{i},Y^{i};Z^{i})-\text{constant} &\geq \E_{p(z^{i},y^{i},x^{i})} \left[ \log p_{\theta}(y^{i}|x^{i},z^{i})\right] \nonumber\\
    &+\E_{p(z^{i},x^{i})} \left [ \log p_{\theta}(x^{i}|z^{i}) \right]\nonumber\\
    &= I_v(X^{i},Y^{i};Z^{i}).
\end{align} 
Hence, the maximization of $I(X^{i},Y^{i};Z^{i})$ can be achieved by maximizing $I_v(X^{i},Y^{i};Z^{i})$.
% Hence, we can achieve the maximization of $I(X^{i},Y^{i};Z^{i})$ by maximizing $I_v(X^{i},Y^{i};Z^{i})$. 
We assume the variational distribution $p_{\theta}(y^{i}|z^{i},x^{i})$ and $p_{\theta}(x^{i}|z^{i})$  as the Gaussion distribution. 
% Thus, the first term of $I_v(X^{i},Y^{i};Z^{i})$ is the negative log-likelihood of the prediction of $Y^{i}$ given $Z^{i}$ and $X^{i}$, and the second term aims to the reconstruction of $X^{i}$ given $Z^{i}$.
Consequently, the first term of $I_v(X^{i},Y^{i};Z^{i})$ represents the negative log-likelihood of predicting $Y^{i}$ given $Z^{i}$ and $X^{i}$, while the second term aims to reconstruct $X^{i}$ given $Z^{i}$.







% \sout{\By using the empirical data distribution following~\citep{alemi2016deep}, we have the approximated lower bound:}
% \begin{equation}
%     \begin{aligned}
%     I(X^{i},Y^{i};Z^{i})  \geq I_{a}(X^{i},Y^{i};Z^{i}) &=\frac{1}{N} \sum_{n=1}^{n} \left [ \int p(z^{i}|x,x^{i})p(y^{i}|x,x^{i})p(x^{i}|x)\log p_{\theta}(y^{i}|x^{i},z^{i}) dz^{i} dx^{i} dy^{i} \right \\ 
%      &\left  + \int p(z^{i}|x,x^{i}) p(x^{i}|x) \log p_{\theta}(x^{i}|z^{i}) dz^{i} dx^{i}  \right] \\
%     \end{aligned}
% \end{equation}


%We approximate $p(x,y)$ using the empirical data distribution $p(x,y)=\sum_{n=1}^{N}\delta_{x_{n}}(x)\delta_{y_{n}}(y)$ following~\cite{alemi2016deep}

\textbf{Upper bound for} $I(X^{o};Z^{i})$. Next, to minimize the MI between the latent representation $Z^{i}$ and historical series $X^{o}$, 
%given $X^{i}$, 
we adopt the sampled vCLUB as defined in~\cite{cheng2020club}:
\begin{equation}
    I_{v}(X^{o};Z^{i})=\frac{1}{N} \sum_{n=1}^{N} \left [  \log q_{\theta}(z_{n}^{i}|x_{n}^{o})- \log q_{\theta}(z_{n}^{i}|x^{o}_{k'_{n}}) \right ],
\end{equation}
where $(z_{n}^{i},x^{o}_{k'_{n}})$ represents a negative pair and $k_{n}'$ is uniformly selected from indices $\{1,2,...N\}$. 
% Thus we can minimize $I(X^{o}; Z^{i})$ by minimizing $I_{v}(X^{o};Z^{i})$.
By minimizing $I_{v}(X^{o};Z^{i})$, we can effectively minimize $I(X^{o}; Z^{i})$. 
It enables the model to extract relevant cross-variable information while eliminating irrelevant information.

Finally, We can convert the intractable objective function $\mathcal{R}_{IB}^{i}$ of all {channels} in Eq.~\ref{ib} as:

\begin{equation}
\begin{aligned}
    \mathcal{L}_{IB}&= \frac{1}{C} \sum_{i=1}^{C}\left[-I_v(X^{i},Y^{i};Z^{i}) + \beta I_{v}(X^{o};Z^{i}) \right] \nonumber\\
    &{\geq -\frac{1}{C}\sum_{i=1}^{C}\mathcal{R}_{IB}^{i}}=-\mathcal{R}_{IB}.
\end{aligned}
\end{equation}
The objective function $\mathcal{L}_{IB}$ is a tractable approximation of the original objective function $\mathcal{R}_{IB}$, we can effectively maximize $\mathcal{R}_{IB}^{i}$ by minimizing $\mathcal{L}_{IB}$.

\subsection{Temporal Correlation Aware Modeling}
\label{approach:TAM}
% \begin{wrapfigure}{r}{0.55\textwidth}
% \vspace*{-20pt}
% \centering
% \includegraphics[width=0.50\columnwidth]{figure/ms.pdf}
% \caption{Architecture of \ms \xspace with 4x dowmsampling. We downsample the target series and forecasted series utilizing single-forecaster into four sub-sequences, respectively. And then we maximize the mutual information between the adjacent sub-sequences of forecasted series and target series.}
% \label{fig:ms}
% \end{wrapfigure}

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{icml2024/figure/ms.pdf}}
\caption{Architecture of \ms \xspace with 4$\times$ dowmsampling. We downsample the target series and forecasted series utilizing single-forecaster into four sub-sequences, respectively. And then we maximize the mutual information between the adjacent sub-sequences of forecasted series and target series.}
\label{fig:ms}
\end{center}
\vskip -0.2in
\end{figure}



% To alleviate the error accumulation effects, previous works~\citep{nie2022time,zeng2022transformers,zhou2021informer,zhang2023crossformer} use a single-step forecaster which is usually a fully-connected network to predict the future series. Different from auto-regressive forecaster, single-step forecaster assumes the predicted future time steps are independent of each other given the historical time series. Then, the training objective of the single-step forecaster can be expressed as follows :

Previous works~\citep{nie2022time,zeng2022transformers,zhou2021informer,zhang2023crossformer} have attempted to alleviate error accumulation effects by using a single-step forecaster, which is typically implemented as a fully-connected network, to predict future time series. Unlike auto-regressive forecasters, which consider dependencies between predicted future time steps, the single-step forecaster assumes that the predicted time steps are independent of each other given the historical time series. Consequently, the training objective of the single-step forecaster can be expressed as:
\begin{equation}
p(y^{i}|z^{i},x^{i})=\prod_{j=1}^{P}p(y^{i}_{j}|z^{i},x^{i})
\end{equation}
%\begin{equation}
%    I(Y^{i};X^{i},Z^{i})=\prod_{j=1}^{P} I(Y^{i}_{p}|X^{i},Z^{i})
%\end{equation}

%Although the single-step forecaster performs better compared with  the auto-regressive forecaster, it does not model the temporal correlations of different timesteps in the target series.
% Although the single-step forecaster outperforms the auto-regressive forecaster, it fails to model the temporal correlations of different timesteps in the target series.
% In contrast to NLP, time series data is a low-density information source~\citep{lin2023petformer}, and one unique property of time series is that the temporal relations (e.g., the trend and the seasonal) between downsampling adjacent sub-sequences are largely preserved~\citep{liu2022scinet}. Based on the above observations, we propose {\ms} \xspace which improves the correlation of predicted future time steps by iteratively down-samples and optimizes mutual information between consecutive sub-sequences of both the forecasted and target series. 
%downsampling maximizing the mutual information between the adjacent sub-sequences of the predicted series and the target series.
%Therefore, to enhance the correlation of predicted future time steps, we propose \textcolor{blue}{method} which downsampling and maximizing the Mutual Information of adjacent sub-sequences.

While the single-step forecaster outperforms the auto-regressive forecaster, it falls short in capturing the temporal correlations among different timesteps in the target series. In contrast to NLP, time series data is considered a low-density information source~\cite{lin2023petformer}. One unique property of time series data is that the temporal relations, such as trends and seasonality, are similar between downsampling adjacent sub-sequences~\cite{liu2022scinet}. Building upon the above observation, we propose {\ms} \xspace to enhance the correlation of predicted future time steps by iteratively down-sampling the time series and optimizing the mutual information between consecutive sub-sequences of both the forecasted and target series. Next, we will introduce \ms \xspace in detail.

{After extracting cross-variable feature $Z^{i}$ as described in Sec~\ref{approach:CAM}, we first generate $\hat{Y^{i}}$ using a single-step forecaster that leverages the historical data of the i-th channel $X^{i}$ and $Z^{i}$ }.
The forecasted series $\hat{Y}$ and target series $Y$ are then downsampled $N$ times. For the n-th ($n \leq N$) downsampling, we generate $m$ sub-sequences $\hat{Y}= \{ \hat{Y}_{1},...,\hat{Y}_{m} \}$,$Y=\{ Y_{1},...,Y_{m} \}$, where $m=2^{n}$ and $\hat{Y}_{j} \in R^{\frac{P}{2^{n}} \times C}$.
Next, we aim to maximize the mutual information $\hat{Y}_{j}^{i}$ and $Y_{j-1}^{i}$, $Y_{j+1}^{i}$, given $X^{i}$, where $1<j<m$. This is achieved by calculating $\mathcal{L}_{n}$ for the $n$-the downsampling:
% Next, we maximize the mutual information between $\hat{Y}_{j}^{i}$ and $Y_{j-1}^{i}$, $Y_{j+1}^{i}$, given $X^{i}$, where $1<j<m$. Therefore, the loss function of $n$-th downsampling can be calculated as:
\begin{equation}
\begin{aligned}
    \mathcal{L}_{n}&=-\frac{1}{mC} \sum_{i=1}^{C} \Big[  I(Y_{2}^{i};\hat{Y}_{1}^{i}|X^{i})+I(Y_{m-1}^{i};\hat{Y}_{m}^{i}|X^{i}) \nonumber \\
    &+ \sum_{j=2}^{m-1} I(Y_{j-1}^{i};\hat{Y}_{j}^{i}|X^{i}) +I(Y_{j+1}^{i};\hat{Y}_{j}^{i}|X^{i})  \Big].
\end{aligned}
\end{equation}

We also introduce the variational lower bound for $I(Y^{i}_{j-1};\hat{Y}_{j}^{i}|X^{i})$, which is as follows (More details are shown in Appendix~\ref{sec:a.3}):
% And the variational lower bound of $I(Y^{i}_{j-1};\hat{Y}_{j}^{i}|X^{i})$ is as follows (More details are shown in Appendix~\ref{sec:a2.2}):
\begin{equation}
    I(Y^{i}_{j-1};\hat{Y}_{j}^{i}|X^{i}) \geq \E_{p(y_{j-1}^{i},\hat{y}_{j}^{i},x^{i})} \left[ p_{\theta}(y_{j-1}^{i}|\hat{y}_{j}^{i},x^{i}) \right].
\end{equation}

Furthermore, considering the efficiency, we make the assumption that the time steps of a sub-sequence are independent given the adjacent sub-sequence. 
As a result, we can simplify the mutual information term, $I(Y^{i}_{j-1};\hat{Y}_{j}^{i}|X^{i})$ as $I(Y^{i}_{j-1};\hat{Y}_{j}^{i}|X^{i})= \sum_{k=1}^{\frac{P}{2^{n}}} \left[ I(Y^{i}_{j-1,k};\hat{Y}_{j}^{i}|X^{i}) \right]$. This allows us to generate the entire sub-sequence in a single step without requiring auto-regression.
% Therefore, $I(Y^{i}_{j-1};\hat{Y}_{j}^{i}|X^{i})$ can be simplified as $I(Y^{i}_{j-1};\hat{Y}_{j}^{i}|X^{i})= \sum_{k=1}^{\frac{P}{2^{n}}} \left[ I(Y^{i}_{j-1,k};\hat{Y}_{j}^{i}|X^{i}) \right]$ and we can generate the entire sub-sequence in a single step without auto-regression.

For the n-th downsampling, \ms \xspace will generate $2\times(2^{n}-1)$ sub-sequences denoted as $\hat{Y}'=\{ \hat{Y}_{1}^{r}, \hat{Y}_{2}^{l},\hat{Y}_{2}^{r},..., \hat{Y}_{m}^{l}\}$.
These sub-sequences, except for the ones and the ends, are predicted by their left and right adjacent sub-sequences respectively. We then splice these $2\times(2^{n}-1)$ sub-sequences into a new series $\hat{Y}_{n}=\{ \hat{Y}_{1}^{r}, \frac{\hat{Y}_{2}^{l}+\hat{Y}_{2}^{r}}{2},...,\hat{Y}_{m}^{l}\}$. After $N$ downsamplings, we have generated $N+1$ series. We use these $N+1$ series as the final forecasting results, resulting in the following loss function:

% these sub-sequences that are not at ends are predicted by its left and right adjacent sub-sequences respectively. We splice these $2\times(2^{n}-1)$ sub-sequences into a new series $\hat{Y}_{n}=\{ \hat{Y}_{1}^{r}, \frac{\hat{Y}_{2}^{l}+\hat{Y}_{2}^{r}}{2},...,\hat{Y}_{m}^{l}\}$.
% After $N$ times downsampling, we have generated $N+1$ series. And we use these $N+1$ series as the final forecasting results, thus we have the following loss function:
\begin{equation}
    \mathcal{L}_{p}= ||Y-(\lambda \sum_{n=1}^{N}{\frac{\hat{Y}_{n}}{N}}+(1-\lambda)\hat{Y})||_{2}^{2}
\end{equation}

%\textcolor{blue}{Compared with single-step forecaster that generate multi-step predictions while ignoring the correlation between predicted series, \ms explicitly models the correlation of predicted future time steps by iteratively down-samples and optimizes the mutual information between between consecutive sub-sequences of both the forecasted and target series which allows the model to better establish representations of future sequences, thereby enhancing the model's predictive performance.}

{In contrast to single-step forecasters that generate multi-step predictions without considering the correlation between the predicted series, our proposed method, referred to as \ms, 
explicitly models the correlation of predicted future time steps and allows to generate more accurate and coherent predictions. 
% It achieves this by iteratively down-sampling and optimizing the mutual information between consecutive sub-sequences of both the forecasted and target series. This approach allows the model to establish more accurate representations of future sequences, thereby enhancing the overall predictive performance. By incorporating the correlation between predicted time steps, \ms \xspace considers the temporal dependencies within the forecasted series and captures the underlying patterns in the data. This iterative down-sampling and mutual information optimization procedure ensures that the model effectively leverages the available information to generate more accurate and coherent predictions.
}

Integrating \mf \xspace and \ms, the total loss of \framework \xspace  can be written as :
\begin{equation}
    \mathcal{L}_{total}=\mathcal{L}_{IB} + \sum_{n=1}^{N} \mathcal{L}_{n}+\mathcal{L}_{p}.
\end{equation}

%\begin{equation}
%    \mathcal{L}_{k}=-\frac{1}{MC}\sum_{i=1}^{C}\sum_{j=2}^{P/k}I(Y_{j}^{i};Y_{j-1}^{i}|X^{i})
%\end{equation}
%\begin{equation}
%    \mathcal{L}_{k}=-\frac{1}{MC}\sum_{i=1}^{C} \left [ I(\hat{Y}^{i}_{1};Y^{i}_{2};X^{i}) +I(\hat{Y}^{i}_{\frac{P}{2^{k}}},Y^{i}_{\frac{P}{2^{k}}-1}|X^{i})+ \sum_{j=2}^{\frac{P}{2^{k}}-1}I(\hat{Y}^{i}_{j},Y^{i}_{j-1}|X^{i})+I(\hat{Y}^{i}_{j};Y^{i}_{j+1}|X^{i}) \right ]
%\end{equation}

%it does not establish the correlation between future time steps, thus makes the model unable to learn the joint probability distribution of the future series. Therefore, we 


%Instead of autoregressive property~\cite{germain2015made}, we propose a downsampling property to construct the joint probability distribution.
%\begin{wrapfigure}[8]{r}{30em}
%    \begin{center}
%        \includegraphics[width=0.6\linewidth]{figure/down-sampling.pdf}
%        \caption{fig:1}
%        \label{fig:down_sampling}
%    \end{center}
%\end{wrapfigure}



==> icml2024/section/conclusion.tex <==
\section{Conclusion}
This paper focus on two key factors in MTSF: temporal correlation and cross-variable correlation. To utilize the cross-variable correlation while eliminating the superfluous information, we introduce \textbf{C}ross-Variable Decorrelation \textbf{A}ware \textbf{M}odeling (\mf). In addition, we also propose \textbf{T}emporal Correlation \textbf{A}ware \textbf{M}odeling (\ms) to model temporal correlations of predicted series. Integrating \mf \xspace and \ms, we build a novel time series modeling framework for MTSF termed \framework . Extensive experiments on various real-world MTSF datasets demonstrate the effectiveness of our framework.

==> icml2024/section/experiment.tex <==
\section{Experiments}
\begin{figure*}[h!]
	\centering
	\subfloat[Informer on ETTh1]{
		\begin{minipage}[t]{0.25\linewidth}
			\centering
			\includegraphics[width=1.54in]{figure/Informer_h.pdf}\\
			\vspace{0.01cm}
		\end{minipage}%
	}%
	\subfloat[Stationary on ETTh1]{
		\begin{minipage}[t]{0.25\linewidth}
			\centering
			\includegraphics[width=1.5in]{figure/Stationary_h.pdf}\\
			\vspace{0.01cm}
		\end{minipage}%
	}%
	\subfloat[PatchTST on ETTh1]{
		\begin{minipage}[t]{0.25\linewidth}
			\centering
			\includegraphics[width=1.5in]{figure/patchtst_h.pdf}\\
			\vspace{0.01cm}
		\end{minipage}%
	}%
 \subfloat[RMLP on ETTh1]{
		\begin{minipage}[t]{0.25\linewidth}
			\centering
			\includegraphics[width=1.5in]{figure/rmlp_h.pdf}\\
			\vspace{0.01cm}
		\end{minipage}%
	}%
	\centering
	\caption{{Evaluation on hyper-parameter $\beta$ and $\lambda$. We evaluate the impact of $\beta$ with Informer and Stationary on the ETTh1 dataset, we also evaluate $\lambda$ with PatchTST and RMLP on the ETTh1 dataset.}}
	\vspace{-0.2cm}
	\label{fig:ablation_beta}
\end{figure*}
\begin{table*}[h!]\small
\caption{Multivariate long-term series forecasting results on Channel-mixing models with different prediction lengths $O \in \{96,192,336,720\}$. We set the input length $I$ as 96 for all the models. The best result is indicated in bold font. {\textit{Avg} is averaged from all four prediction lengths.
and \textit{Pro} means the relative MSE or MAE reduction. 
(See Table~\ref{tab:ablation_dependent} for the full results.)}}
    \centering
    \tabcolsep=0.15cm
    \begin{tabular}{c|c|cccc|cccc|cccc}
    
    \hline
    \multicolumn{2}{c|}{\multirow{2}{*}{Models}} & \multicolumn{4}{c|}{Informer} & \multicolumn{4}{c|}{Stationary} & \multicolumn{4}{c}{Crossformer} \\
    
    \multicolumn{2}{c|}{} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c|}{w/Ours} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c|}{w/Ours} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{w/Ours} \\
    \hline
    \multicolumn{2}{c|}{Metric} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\
    \hline
    % \multirow{4}{*}{\rotatebox{90}{ETTh1}} 
    % & 96 & 0.865 & 0.713 & \textbf{0.381} & \textbf{0.394} & 0.598 & 0.498 & \textbf{0.375} & \textbf{0.388} & 0.457 & 0.463 & \textbf{0.379} & \textbf{0.392} \\
    % & 192 & 1.008 & 0.792 & \textbf{0.435} & \textbf{0.430} & 0.602 & 0.520 & \textbf{0.425} & \textbf{0.417} & 0.635 & 0.581 & \textbf{0.433} & \textbf{0.427} \\
    % & 336 & 1.107 & 0.809 & \textbf{0.485} & \textbf{0.461} & 0.677 & 0.573 & \textbf{0.463} & \textbf{0.436} & 0.776 & 0.667 & \textbf{0.482} & \textbf{0.458} \\
    % & 720 & 1.181 & 0.865 & \textbf{0.534} & \textbf{0.524} & 0.719 & 0.597 & \textbf{0.463} & \textbf{0.459} & 0.861 & 0.725 & \textbf{0.529} & \textbf{0.517} \\
    % \hline
    % & Avg & 1.040 & 0.794 & \textbf{0.458} & \textbf{0.452} & 0.649 & 0.547 & \textbf{0.431} & \textbf{0.425} & 0.682 & 0.609 & \textbf{0.455} & \textbf{0.448} \\
    % \hline 
    % & Pro & - & - & \textbf{55.9\%} & \textbf{43.0\%} & - & - & \textbf{33.5\%} & \textbf{22.3\%} & - & - & \textbf{33.2\%} & \textbf{26.4\%} \\
    % \hline
    % \multirow{4}{*}{\rotatebox{90}{{ETTh2}}} 
    % & 96 & 3.755 & 1.525 & \textbf{0.336} & \textbf{0.390} & 0.362 & 0.393 & \textbf{0.286} & \textbf{0.335} & 0.728 & 0.615 & \textbf{0.333} & \textbf{0.386} \\
    % & 192 & 5.602 & 1.931 & \textbf{0.468} & \textbf{0.470} & 0.481 & 0.453 & \textbf{0.371} & \textbf{0.388} & 0.898 & 0.705 & \textbf{0.455} & \textbf{0.453} \\
    % & 336 & 4.721 & 1.835 & \textbf{0.582} & \textbf{0.534} & 0.524 & 0.487 & \textbf{0.414} & \textbf{0.425} & 1.132 & 0.807 & \textbf{0.554} & \textbf{0.513} \\
    % & 720 & 3.647 & 1.625 & \textbf{0.749} & \textbf{0.620} & 0.512 & 0.494 & \textbf{0.418} & \textbf{0.437} & 4.390 & 1.795 & \textbf{0.757} & \textbf{0.619} \\
    % \hline
    % & Avg & 4.431 & 1.729 & \textbf{0.534} & \textbf{0.504} & 0.470 & 0.457 & \textbf{0.372}& \textbf{0.396} & 1.787 & 0.981 & \textbf{0.525} & \textbf{0.493} \\
    % \hline 
    % & Pro & - & - & \textbf{87.9\%} & \textbf{70.9\%} & - & - & \textbf{20.9\%} & \textbf{13.3\%} & - & - & \textbf{70.6\%} & \textbf{49.7\%} \\
    % \hline
    % \multirow{4}{*}{\rotatebox{90}{ETTm1}} 
    % & 96 & 0.672 & 0.571 & \textbf{0.326} & \textbf{0.367} & 0.396 & 0.401 & \textbf{0.326} & \textbf{0.362} & 0.385 & 0.409 & \textbf{0.323} & \textbf{0.362} \\
    % & 192 & 0.795 & 0.669 & \textbf{0.371} & \textbf{0.391} & 0.471 & 0.436 & \textbf{0.366} & \textbf{0.379} & 0.459 & 0.478 & \textbf{0.366} & \textbf{0.386} \\
    % & 336 & 1.212 & 0.871 & \textbf{0.408} & \textbf{0.416} & 0.517 & 0.464 & \textbf{0.392} & \textbf{0.398} & 0.649 & 0.583 & \textbf{0.403} & \textbf{0.414} \\
    % & 720 & 1.166 & 0.823 & \textbf{0.482} & \textbf{0.464} & 0.664 & 0.527 & \textbf{0.455} & \textbf{0.434} & 0.756 & 0.669 & \textbf{0.473} & \textbf{0.460} \\
    % \hline
    % & Avg & 0.961 & 0.733 & \textbf{0.396} & \textbf{0.409} & 0.512 & 0.457 & \textbf{0.384} & \textbf{0.393} & 0.562 & 0.534 & \textbf{0.391} & \textbf{0.405} \\
    % \hline 
    % & Pro & - & - & \textbf{58.7\%} & \textbf{44.2\%} & - & - & \textbf{25.0\%} & \textbf{14.0\%} & - & - & \textbf{30.4\%} & \textbf{24.1\%} \\
    % \hline
    \multirow{4}{*}{\rotatebox{90}{ETTm2}} 
    & 96 & 0.365 & 0.453 & \textbf{0.187} & \textbf{0.282} & 0.201 & 0.291 & \textbf{0.175} & \textbf{0.256} & 0.281 & 0.373 & \textbf{0.186} & \textbf{0.281} \\
    & 192 & 0.533 & 0.563 & \textbf{0.277} & \textbf{0.351} & 0.275 & 0.335 & \textbf{0.238} & \textbf{0.297} & 0.549 & 0.520 & \textbf{0.269} & \textbf{0.341} \\
    & 336 & 1.363 & 0.887 & \textbf{0.380} & \textbf{0.420} & 0.350 & 0.377 & \textbf{0.299} & \textbf{0.336} & 0.729 & 0.603 & \textbf{0.356} & \textbf{0.396} \\
    & 720 & 3.379 & 1.338 & \textbf{0.607} & \textbf{0.549} & 0.460 & 0.435 & \textbf{0.398} & \textbf{0.393} & 1.059 & 0.741 & \textbf{0.493} & \textbf{0.482} \\
    \hline
    & Avg & 1.410 & 0.810 & \textbf{0.362} & \textbf{0.400} & 0.321 & 0.359 & \textbf{0.277} & \textbf{0.320} & 0.654 & 0.559 & \textbf{0.326} & \textbf{0.375} \\
    \hline 
    & Pro & - & - & \textbf{74.3\%} & \textbf{50.6\%} & - & - & \textbf{13.7\%} & \textbf{10.8\%} & - & - & \textbf{50.1\%} & \textbf{32.9\%} \\
    \hline
    \multirow{4}{*}{\rotatebox{90}{Weather}} 
    & 96 & 0.300 & 0.384 & \textbf{0.179} & \textbf{0.249} & 0.181 & 0.230 & \textbf{0.166} & \textbf{0.213} & 0.158 & 0.236 & \textbf{0.149} & \textbf{0.218} \\
    & 192 & 0.598 & 0.544 & \textbf{0.226} & \textbf{0.296} & 0.286 & 0.312 & \textbf{0.218} & \textbf{0.260} & 0.209 & 0.285 & \textbf{0.202} & \textbf{0.272} \\
    & 336 & 0.578 & 0.523 & \textbf{0.276} & \textbf{0.334} & 0.319 & 0.335 & \textbf{0.274} & \textbf{0.300} & 0.265 & 0.328 & \textbf{0.256} & \textbf{0.313} \\
    & 720 & 1.059 & 0.741 & \textbf{0.332} & \textbf{0.372} & 0.411 & 0.393 & \textbf{0.351} & \textbf{0.353} & 0.376 & 0.397 & \textbf{0.329} & \textbf{0.366} \\
    \hline
    & Avg & 0.633 & 0.548 & \textbf{0.253} & \textbf{0.312} & 0.299 & 0.317 & \textbf{0.252} & \textbf{0.281} & 0.252 & 0.311 & \textbf{0.234} & \textbf{0.292} \\
    \hline 
    & Pro & - & - & \textbf{60.0\%} & \textbf{43.0\%} & - & - & \textbf{15.7\%} & \textbf{11.3\%} & - & - & \textbf{7.1\%} & \textbf{6.1\%} \\
    \hline
    \multirow{4}{*}{\rotatebox{90}{Traffic}} 
    & 96 & 0.719 & 0.391 & \textbf{0.505} & \textbf{0.348} & 0.599 & 0.332 & \textbf{0.459} & \textbf{0.311} & 0.609 & 0.362 & \textbf{0.529} & \textbf{0.334} \\
    & 192 & 0.696 & 0.379 & \textbf{0.521} & \textbf{0.354} & 0.619 & 0.341 & \textbf{0.475} & \textbf{0.315} & 0.623 & 0.365 & \textbf{0.519} & \textbf{0.327} \\
    & 336 & 0.777 & 0.420 & \textbf{0.520} & \textbf{0.337} & 0.651 & 0.347 & \textbf{0.486} & \textbf{0.319} & 0.649 & 0.370 & \textbf{0.521} & \textbf{0.337} \\
    & 720 & 0.864 & 0.472 & \textbf{0.552} & \textbf{0.352} & 0.658 & 0.358 & \textbf{0.522} & \textbf{0.338} & 0.758 & 0.418 & \textbf{0.556} & \textbf{0.350} \\
    \hline
    & Avg & 0.764 & 0.415 & \textbf{0.524} & \textbf{0.347} & 0.631 & 0.344 & \textbf{0.485} & \textbf{0.320} & 0.659 & 0.378 & \textbf{0.531} & \textbf{0.337} \\
    \hline
    & Pro & - & - & \textbf{31.4\%} & \textbf{16.3\%} & - & - & \textbf{23.1\%} & \textbf{6.9\%} & - & - & \textbf{19.4\%} & \textbf{10.8\%} \\
    \hline
    \multirow{4}{*}{\rotatebox{90}{Electricity}} 
    & 96 & 0.274 & 0.368 & \textbf{0.195} & \textbf{0.300} & 0.168 & 0.271 & \textbf{0.154} & \textbf{0.256} & 0.170 & 0.279 & \textbf{0.150} & \textbf{0.248} \\
    & 192 & 0.296 & 0.386 & \textbf{0.193} & \textbf{0.291} & 0.186 & 0.285 & \textbf{0.163} & \textbf{0.263} & 0.198 & 0.303 & \textbf{0.168} & \textbf{0.263} \\
    & 336 & 0.300 & 0.394 & \textbf{0.206} & \textbf{0.300} & 0.194 & 0.297 & \textbf{0.178} & \textbf{0.279} & 0.235 & 0.328 & \textbf{0.200} & \textbf{0.290} \\
    & 720 & 0.373 & 0.439 & \textbf{0.241} & \textbf{0.332} & 0.224 & 0.316 & \textbf{0.201} & \textbf{0.299} & 0.270 & 0.360 & \textbf{0.235} & \textbf{0.323} \\
    \hline
    & Avg & 0.310 & 0.397 & \textbf{0.208} & \textbf{0.305} & 0.193 & 0.292 &  0.174 & \textbf{0.274} & 0.218 & 0.317 & \textbf{0.188} & \textbf{0.281} \\


    \hline 
    & Pro & - & - & \textbf{32.9\%} & \textbf{23.1\%} & - & - & \textbf{9.8\%}  & \textbf{6.1\%} & - & - & \textbf{13.7\%} & \textbf{11.3\%} \\
    \hline
    \end{tabular}
    \label{tab:main_results_channel_dependent}
\end{table*}
In this section, we extensively evaluate the proposed \framework \xspace on 10 real-world benchmarks using various Channel-mixing and Channel-Independence models,
including state-of-the-art models.

\textbf{Baselines.} In order to demonstrate the versatility of our proposed method, \framework, we evaluate it on various deep-learning-based forecasting models, including several popular baselines as well as the state-of-the-art method.  
% Since our method can be easily applied to deep-learning-based forecasting models, we evaluate \framework \xspace adopted by several popular baselines including the state-of-the-art method. 
For Channel-mixing models, we select Informer~\citep{zhou2021informer}, Non-stationary Transformer~\citep{liu2022non}, denoting as Stationary, and Crossformer~\citep{zhang2023crossformer}. As for Channel-Independence models, we utilize PatchTST~\citep{nie2022time} and also introduce RMLP which consists of two linear layers with ReLU activation and also incorporates reversible instance normalization~\citep{kim2021reversible}. (see Appendix~\ref{baselines} for more details) 
%We set historical length $T=336$ for PatchTST and RMLP, and $T=96$ for other baselines.

\textbf{Datasets.} We extensively include 10 real world datasets in our experiments, including four ETT datasets (ETTh1, ETTh2, ETTm1, ETTm2)~\cite{zhou2021informer}. Electricity, Weather, Traffic~\cite{chen2021autoformer}, and PEMS covering energy, transportation and weather domains (See Appendix~\ref{sec:dataset_details} for more details on the datasets). We follow the standard protocol that divides each dataset into the training, validation, and testing subsets according to the chronological order. The split ratio is 6:2:2 for the ETT dataset and 7:1:2 for others.

% We evaluate the performance of \framework \xspace in nine widely-used real-world datasets. Here is a detailed description of these datasets. (1) The ETT~\citep{zhou2021informer} (Electricity Transformer Temperature) dataset contains two years of data from two separate countries in China with intervals of 1-hour level (ETTh) and 15-minute level (ETTm) collected from electricity transformers. Each time step contains six power load features and oil temperature. (2) The Electricity \footnote[1]{ \href{https://archive.ics.uci.edu/ml/datasets/ElectricityLoadDiagrams20112014}{https://archive.ics.uci.edu/ml/datasets/ElectricityLoadDiagrams20112014.}} dataset describes 321 clients' hourly electricity consumption  from 2012 to 2014. (3) The Traffic \footnote[2]{\href{http://pems.dot.ca.gov}{http://pems.dot.ca.gov.}} dataset contains the road occupancy rates from various sensors on San Francisco Bay area freeways, which is provided by California Department of Transportation. (4) the Weather \footnote[3]{\href{https://www.bgc-jena.mpg.de/wetter/}{https://www.bgc-jena.mpg.de/wetter/.}} dataset contains 21 meteorological indicators collected at around 1,600 landmarks in the United States. (5)The PEMS~\citep{chen2001freeway} (PEMS03, PEMS04, and PEMS08) measures the highway traffic of California in real-time every 30 seconds. We follow the standard protocol that divides each dataset into the training, validation, and testing subsets according to the chronological order. The split ratio is 6:2:2 for the ETT dataset and 7:1:2 for others.

%\textbf{Implementation Details.}

\subsection{Main Results}

Table~\ref{tab:main_results_channel_dependent} compares the forecasting accuracy of the Channel-mixing baselines and \framework.
%The results clearly demonstrate that \framework \xspace consistently outperforms all three baselines, Informer, Stationary, and Crossformer, by a significant margin. 
The results clearly demonstrate that \framework \xspace consistently outperforms all three baselines, namely Informer, Stationary, and Crossformer, by a significant margin. This improvement is particularly notable for long sequence predictions, which are generally more challenging and prone to the model relying on irrelevant cross-variable information. \framework \xspace exhibits stable performance, whereas the baselines experience a substantial increase in forecasting error as the prediction length is extended.
%The results show that \framework \xspace consistently outperforms all three baselines, Informer, Stationary, and Crossformer, by a large margin. 
%Moreover, the effectiveness of \framework \xspace is more evident for the long sequence prediction which may be long sequence prediction is more difficult and more likely to lead the model depending on superfluous cross-variable information. \framework \xspace shows a stable performance in contrast to the baselines, which show a high increase in error as prolonging the prediction length. 
For example, on the ETTm2 dataset, when the prediction length increases from 96 to 720, the forecasting error of Informer rises significantly from 0.365 to 3.379. In contrast, \framework \xspace shows a much slight increase in error.
% For example, when the prediction length increases from 96 to 720 on the ETTm2 dataset, the forecasting error of Informer significantly increases from 0.365 to 3.379. In contrast, \framework \xspace shows a much slight increase in error. 
A similar tendency appears with the other prediction lengths, datasets, and baseline models as well. These results demonstrate that \framework \xspace makes the baseline models more robust to prediction target series. 

To gain further insights into why \framework \xspace outperforms baselines, we visualize the testing error for each epoch in Figure~\ref{fig:test_loss}. Overall, \framework \xspace exhibits lower and more stable test errors compared to the baselines. Moreover, the baselines are highly prone to overfitting in the early stages of training, whereas \framework \xspace effectively mitigates this issue.
%Additionally, to study how \framework \xspace can perform better than baselines, we visualize the testing error for each epoch in Figure~\ref{fig:test_loss}. Overall, \framework \xspace shows lower and more stable test errors compared to the baselines. Moreover, the baselines are extremely prone to overfitting in the early stages of training, and \framework \xspace can effectively alleviate this problem.
%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.4]{figure/test_loss.pdf}
%\caption{\textbf{Test error for each training epoch}. We train the baselines and integrated with our \framework \xspace for 50 epochs on ETTh1 when the history and prediction length are both 96.}
%\label{fig:test_loss}
%\end{figure}

\begin{figure*}[h!]
	\centering
	\subfloat[Test error on Informer]{
		\begin{minipage}[t]{0.3\linewidth}
			\centering
			\includegraphics[width=1.76in]{figure/Informer2.pdf}\\
			\vspace{0.015cm}
		\end{minipage}%
	}%
	\subfloat[Test error on Stationary]{
		\begin{minipage}[t]{0.3\linewidth}
			\centering
			\includegraphics[width=1.8in]{figure/Stationary2.pdf}\\
			\vspace{0.02cm}
		\end{minipage}%
	}%
	\subfloat[Test error on Crossformer]{
		\begin{minipage}[t]{0.3\linewidth}
			\centering
			\includegraphics[width=1.8in]{figure/Crossformer.pdf}\\
			\vspace{0.02cm}
		\end{minipage}%
	}%
	\centering
	\caption{\textbf{Test error for each training epoch}. We train the baselines and integrated with our \framework \xspace for 50 epochs on ETTh1 with the history and prediction length are both 96.}
	\vspace{-0.2cm}
	\label{fig:test_loss}
\end{figure*}


\begin{table*}[h!]
    \centering
    \caption{Multivariate long-term series forecasting results on Channel-Independence models with different prediction lengths. We set the input length $I$ as 336 for all the models. The best result is indicated in bold font. See {Table~\ref{tab:main_results_channel_independent_full}} in the Appendix for the full results.}
    \tabcolsep=0.08cm
    \begin{tabular}{ccc|cccc|cccc|cccc}
    \hline
         \multicolumn{2}{c}{\multirow{2}{*}{Models}} & \multirow{2}{*}{Metric} & \multicolumn{4}{c|}{ETTh1} & \multicolumn{4}{c|}{ETTm1} & \multicolumn{4}{c}{Traffic} \\
         \multicolumn{2}{c}{} & & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720  & 96 & 192 & 336 & 720 \\
         \hline
         \multirow{4}{*}{\rotatebox{90}{PatchTST}} & \multirow{2}{*}{Original} & MSE & 0.375 & 0.414 & 0.440 & 0.460 & 0.290 & 0.332 & 0.366 & 0.420 & 0.367 & 0.385 & 0.398 & 0.434 \\
          & & MAE &  0.399 & 0.421 & 0.440 & 0.473 & 0.342 & 0.369 & 0.392 & 0.424 & 0.251 & 0.259 & 0.265 & 0.287 \\
          & \multirow{2}{*}{\textbf{w/Ours}} & MSE & \textbf{0.365} & \textbf{0.403} & \textbf{0.427} & \textbf{0.433} & \textbf{0.283} & \textbf{0.322} & \textbf{0.356} & \textbf{0.407} & \textbf{0.358} & \textbf{0.379} & \textbf{0.391} & \textbf{0.425} \\
          & & MAE  & \textbf{0.389} & \textbf{0.413} & \textbf{0.428} & \textbf{0.453} & \textbf{0.335} & \textbf{0.359} & \textbf{0.382} & \textbf{0.417} & \textbf{0.245} & \textbf{0.254} & \textbf{0.261} & \textbf{0.280} \\ 
          \hline
          \multirow{4}{*}{\rotatebox{90}{RMLP}} & \multirow{2}{*}{Original} & MSE & 0.380 & 0.414 & 0.439 & 0.470 & 0.290 & 0.329 & 0.364 & 0.430 & 0.383 & 0.401 & 0.414 & 0.443 \\
          & & MAE  & 0.401 & 0.421 & 0.436 & 0.471 & 0.343 & 0.368 & 0.390 & 0.426 & 0.269 & 0.276 & 0.282 & 0.309 \\
          & \multirow{2}{*}{\textbf{w/Ours}} & MSE & \textbf{0.367} & \textbf{0.404} & \textbf{0.426} & \textbf{0.439} & \textbf{0.285} & \textbf{0.322} & \textbf{0.358} & \textbf{0.414} & \textbf{0.364} & \textbf{0.384} & \textbf{0.398} & \textbf{0.428} \\
          & & MAE & \textbf{0.391} & \textbf{0.413} & \textbf{0.429} & \textbf{0.459} & \textbf{0.335} & \textbf{0.359} & \textbf{0.381} & \textbf{0.413} & \textbf{0.249} & \textbf{0.258} & \textbf{0.266} & \textbf{0.284} \\
         \hline
    \end{tabular}
    \label{tab:marin_results_channel_independent}
\end{table*}
We also present the forecasting results of Channel-independence baselines in Table~\ref{tab:marin_results_channel_independent}. It is worth noting that \framework \xspace also surpasses Channel-independence baselines, indicating that although Channel-independence models exhibit promising results, incorporating cross-variable features can further enhance their effectiveness. Furthermore, we evaluate \framework \xspace on the PEMS datasets, which consist of variables that exhibit clear geographical correlations. The results in Table~\ref{tab:pems_results} reveal a significant performance gap between PatchTST and RMLP compared to Informer, suggesting that Channel-independence models may not be optimal in scenarios where there are clear correlations between variables. In contrast, our framework exhibits improved performance for both Channel-mixing and Channel-independence models. %({We also verify the effectiveness of \framework \xspace on synthetic data, as show in Appendix~\ref{sec:syn}}).
%As shown in Table~\ref{tab:pems_results}, we observe that PatchTST and RMLP perform worse than Informer by a large margin, which means that Channel-Independent models may be not optimal in all situations, especially when there is a clear correlation between variables. Meanwhile, our framework can improve the performance of Channel-Independent models and Channel-Dependent models.


\begin{table*}[!]
    \centering
    \caption{Multivariate long-term series forecasting results on baselines and PEMS datasets with different prediction lengths. We set the input length $I$ as 336 for all the models. The best result is indicated in bold font. (See {Table~\ref{tab:pems_ablation_results}} for the full results.) }
    \tabcolsep=0.08cm
    \begin{tabular}{ccc|cccc|cccc|cccc}
    \hline
     \multicolumn{2}{c}{\multirow{2}{*}{Models}} & \multirow{2}{*}{Metric} & \multicolumn{4}{c|}{PEMS03} & \multicolumn{4}{c|}{PEMS04} & \multicolumn{4}{c}{PEMS08} \\
     \multicolumn{2}{c}{} & & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 & 96 & 192 & 336 & 720 \\
     \hline
     \multirow{4}{*}{\rotatebox{90}{\footnotesize PatchTST}} & \multirow{2}{*}{Original} & MSE & 0.180 & 0.207 & 0.223 & 0.291 & 0.195 & 0.218 & 0.237 & 0.321 & 0.239 & 0.292 & 0.314 & 0.372 \\
          & & MAE &  0.281 & 0.295 & 0.309 & 0.364 & 0.296 & 0.314 & 0.329 & 0.394 & 0.324 & 0.351 & 0.374 & 0.425 \\
          & \multirow{2}{*}{\textbf{w/Ours}} & MSE & 
          \textbf{0.115} & \textbf{0.154} & \textbf{0.164} & \textbf{0.198} & \textbf{0.110} & \textbf{0.118} & \textbf{0.129} & \textbf{0.149} & \textbf{0.114} & \textbf{0.160} & \textbf{0.177} & \textbf{0.209}\\
          & & MAE & \textbf{0.223} & \textbf{0.251} & \textbf{0.256} & \textbf{0.286} & \textbf{0.221} & \textbf{0.224} & \textbf{0.237} & \textbf{0.261} & \textbf{0.218} & \textbf{0.243} & \textbf{0.241} & \textbf{0.281} \\ 
          \hline
          \multirow{4}{*}{\rotatebox{90}{\footnotesize RMLP}} & \multirow{2}{*}{Original} & MSE & 0.160 & 0.184 & 0.201 & 0.254 & 0.175 & 0.199 & 0.210 & 0.255 & 0.194 & 0.251 & 0.274 & 0.306 \\
          & & MAE  & 0.257 & 0.277 & 0.291 & 0.337 & 0.278 & 0.294 & 0.306 & 0.348 & 0.279 & 0.311 & 0.328 & 0.365 \\
          & \multirow{2}{*}{\textbf{w/Ours}} & MSE & \textbf{0.117} & \textbf{0.159} & \textbf{0.146} & \textbf{0.204} & \textbf{0.103} & \textbf{0.114} & \textbf{0.130} & \textbf{0.154} & \textbf{0.116} & \textbf{0.156} & \textbf{0.175} & \textbf{0.181} \\
          & & MAE & \textbf{0.228} & \textbf{0.252} & \textbf{0.246} & \textbf{0.285} & \textbf{0.211} & \textbf{0.219} & \textbf{0.236} & \textbf{0.264} & \textbf{0.215} & \textbf{0.235} & \textbf{0.242} & \textbf{0.255} \\
          \hline
         % \multirow{4}{*}{\rotatebox{90}{\footnotesize Informer}} & \multirow{2}{*}{Original} & MSE & 0.139 & 0.152 & 0.165 & 0.216 & 0.132 & 0.146 & 0.147 & 0.145 & 0.156 & 0.175 & 0.187 & 0.264 \\
         %  & & MAE  & 0.240 & 0.252 & 0.260 & 0.290 & 0.238 & 0.249 & 0.247 & 0.245 & 0.262 & 0.266 & 0.274 & 0.325 \\
         %  & \multirow{2}{*}{\textbf{w/Ours}} & MSE & \textbf{0.109} & \textbf{0.120} & \textbf{0.144} & \textbf{0.194} & \textbf{0.107} & \textbf{0.124} & \textbf{0.124} & \textbf{0.136} & \textbf{0.099} & \textbf{0.123} & \textbf{0.147} & \textbf{0.196} \\
         %  & & MAE & \textbf{0.216} & \textbf{0.228} & \textbf{0.247} & \textbf{0.282} & \textbf{0.215} & \textbf{0.230} & \textbf{0.231} & \textbf{0.245} & \textbf{0.204} & \textbf{0.224} & \textbf{0.242} & \textbf{0.278} \\
         % \hline
        %   \multirow{4}{*}{\rotatebox{90}{\footnotesize {Stationary}}} & \multirow{2}{*}{Original} & MSE & 0.120 & 0.143 & 0.156 & 0.220 & 0.109 & 0.116 & 0.129 & 0.139 & 0.151 & 0.180 & 0.252 & 0.223 \\
        %   & & MAE  & 0.222 & 0.242 & 0.252 & 0.300 & 0.214 & 0.220 & 0.230 & 0.240 & 0.235 & 0.247 & 0.262 & 0.285 \\
        %   & \multirow{2}{*}{\textbf{w/Ours}} & MSE & \textbf{0.101} & \textbf{0.131} & \textbf{0.153} & \textbf{0.190} & \textbf{0.096} & \textbf{0.114} & \textbf{0.125} & \textbf{0.135} & \textbf{0.103} & \textbf{0.144} & \textbf{0.184} & \textbf{0.217} \\
        %   & & MAE  & \textbf{0.206} & \textbf{0.229} & \textbf{0.245} & \textbf{0.273} & \textbf{0.199} & \textbf{0.217} & \textbf{0.229} & \textbf{0.243} & \textbf{0.200} & \textbf{0.220} & \textbf{0.245} & \textbf{0.278} \\
        %  \hline
        %  \multirow{4}{*}{\rotatebox{90}{\footnotesize {Crossformer}}} & \multirow{2}{*}{Original} & MSE & 0.159 & 0.233 & 0.275 & 0.315 & 0.149 & 0.216 & 0.230 & 0.276 & 0.141 & 0.162 & 0.199 & 0.261 \\
        % & & MAE  &0.270 & 0.319 & 0.351 & 0.383 & 0.261 & 0.320 & 0.324 & 0.369 & 0.253 & 0.269 & 0.306 & 0.355 \\ 
        %  & \multirow{2}{*}{\textbf{w/Ours}} & MSE & 
        % \textbf{0.119} & \textbf{0.166} & \textbf{0.189} & \textbf{0.223} & \textbf{0.114} & \textbf{0.139} & \textbf{0.161} & \textbf{0.171} & \textbf{0.088} & \textbf{0.108} & \textbf{0.134} & \textbf{0.171} \\
        % & & MAE & \textbf{0.217} & \textbf{0.250} & \textbf{0.265} & \textbf{0.293} & \textbf{0.215} & \textbf{0.236} & \textbf{0.258} & \textbf{.275} & \textbf{0.190} & \textbf{0.206} & \textbf{0.222} & \textbf{0.251} \\
        %  \hline
        
    \end{tabular}
    \label{tab:pems_results}
\end{table*}

\subsection{Ablation Study}
\begin{table*}[!]\normalsize
\centering
\tabcolsep=0.15cm
\caption{Component ablation of \framework. We set the input length $I$ as 336 for PatchTST and 96 for Informer. The best results are in \textbf{bold} and the second best are \underline{underlined}. (See {Table~\ref{tab:ablation_dependent}} and {Table~\ref{tab:ablation_independent}} in the Appendix for the full ablation results.)}
\begin{tabular}{cc|cccccc|cccccc}
\hline
     \multicolumn{2}{c|}{\multirow{2}{*}{Models}} & \multicolumn{6}{c|}{Informer} & \multicolumn{6}{c}{PatchTST} \\
     \multicolumn{2}{c|}{} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{+\ms} & \multicolumn{2}{c|}{+\framework} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{+\ms} & \multicolumn{2}{c}{+\framework} \\
     \hline
     \multicolumn{2}{c|}{Metric} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\
     \hline 
    %  \multirow{4}{*}{\rotatebox{90}{ETTh1}} 
    %  & 96 & 0.865 & 0.713 & \underline{0.598} & \underline{0.565} & \textbf{0.381} & \textbf{0.394} & 0.375 & 0.399 & \underline{0.367}& \underline{0.391} & \textbf{0.365} & \textbf{0.389} \\
    % &192 & 1.008 & 0.792 & \underline{0.694} & \underline{0.640} & \textbf{0.435} & \textbf{0.430} & 0.414 & 0.421 &\underline{0.405} &\underline{0.414} & \textbf{0.403} & \textbf{0.413} \\ 
    % &336 & 1.107 & 0.809 & \underline{0.853}& \underline{0.719} & \textbf{0.485} & \textbf{0.461} & 0.440 & 0.440 & \underline{0.429} & \underline{0.430} & \textbf{0.427} & \textbf{0.428} \\ 
    % &720 & 1.181 & 0.865 & \underline{0.914} & \underline{0.741} & \textbf{0.534} & \textbf{0.524} & 0.460 & 0.473 & \underline{0.435} & \underline{0.455} & \textbf{0.433} & \textbf{0.453} \\ 
    % \hline
       
       \multirow{4}{*}{\rotatebox{90}{ETTm1}} 
       & 96 & 0.672 & 0.571 & \underline{0.435} & \underline{0.444} & \textbf{0.335} & \textbf{0.369} & 0.290 & 0.342 & \underline{0.286} & \underline{0.337} & \textbf{0.283} & \textbf{0.335} \\
      & 192 & 0.795 & 0.669 & \underline{0.473} & \underline{0.467} & \textbf{0.380} & \textbf{0.390} & 0.332 & 0.369 & \underline{0.326} & \underline{0.366} & \textbf{0.322} & \textbf{0.363} \\
      & 336 & 1.212 & 0.871 & \underline{0.545} & \underline{0.518} & \textbf{0.423} & \textbf{0.426} & 0.366 & 0.392 & \underline{0.359} & \underline{0.388} & \textbf{0.356} & \textbf{0.385} \\
      & 720 & 1.166 & 0.823 & \underline{0.669} & \underline{0.589} & \textbf{0.505} & \textbf{0.480} & 0.420 & 0.424 & \underline{0.408} & \textbf{0.413} & \textbf{0.407} & \underline{0.417} \\
      \hline
       \multirow{4}{*}{\rotatebox{90}{Weather}} 
       &  96 & 0.300 & 0.384 & \underline{0.277} & \underline{0.354} & \textbf{0.179}& \textbf{0.249} & 0.152 & 0.199 & \underline{0.149} & \underline{0.197} & \textbf{0.144} & \textbf{0.194} \\
        &192 & 0.598 & 0.544 & \underline{0.407} & \underline{0.447} & \textbf{0.226} & \textbf{0.296} & 0.197 & 0.243 & \underline{0.192} & \textbf{0.238} & \textbf{0.189} & \textbf{0.238} \\ 
        &336 & 0.578 & 0.523 & \underline{0.529} & \underline{0.520}& \textbf{0.276} & \textbf{0.334} & 0.250 & 0.284 & \underline{0.247}& \underline{0.280} & \textbf{0.239} & \textbf{0.279} \\ 
       &720 & 1.059 & 0.741 & \underline{0.951} & \underline{0.734} & \textbf{0.332} & \textbf{0.372} & \underline{0.320} & 0.335 & 0.321 & \underline{0.332} & \textbf{0.312} & \textbf{0.331} \\  
       \hline
      \label{tab:ablation}
\end{tabular}
\end{table*}
In our approach, there are two components: \mf \xspace and \ms. To investigate the effectiveness of these components, we conduct an ablation study on the ETTm1 and Weather datasets with Informer and PatchTST. \textbf{+\ms} means that we add \ms \xspace to these baselines and \textbf{+\framework} means that we add both \mf \xspace and \ms \xspace to baselines. 
%We analyze the results shown in Table~\ref{tab:ablation}. 
The results of this ablation study are summarized in Table~\ref{tab:ablation}.
Compared to baselines using the single-step forecaster, \ms \xspace performs better in most settings, which indicates the importance of cross-time correlation. For Channel-mixing models, we find that \framework \xspace can significantly enhance their performance and effectively alleviate the issue of overfitting. For Channel-Independence models, \framework \xspace still improves their performance, which indicates that correctly establishing the dependency between variables is an effective way to improve performance.

% \begin{table*}[ht]\normalsize
% \centering
% \tabcolsep=0.15cm
% \caption{Component ablation of \framework. We set the input length $I$ as 336 for PatchTST and 96 for Informer. The best results are in \textbf{bold} and the second best are \underline{underlined}. (See \textcolor{blue}{Table~\ref{tab:ablation_dependent}} and \textcolor{blue}{Table~\ref{tab:ablation_independent}} in the Appendix for the full ablation results.)}
% \begin{tabular}{cc|cccccc|cccccc}
% \hline
%      \multicolumn{2}{c|}{\multirow{2}{*}{Models}} & \multicolumn{6}{c|}{Informer} & \multicolumn{6}{c}{PatchTST} \\
%      \multicolumn{2}{c|}{} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{+\ms} & \multicolumn{2}{c|}{+\framework} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{+\ms} & \multicolumn{2}{c}{+\framework} \\
%      \hline
%      \multicolumn{2}{c|}{Metric} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\
%      \hline 
%      \multirow{4}{*}{\rotatebox{90}{ETTh1}} 
%      & 96 & 0.865 & 0.713 & \underline{0.598} & \underline{0.565} & \textbf{0.381} & \textbf{0.394} & 0.375 & 0.399 & \underline{0.367}& \underline{0.391} & \textbf{0.365} & \textbf{0.389} \\
%     &192 & 1.008 & 0.792 & \underline{0.694} & \underline{0.640} & \textbf{0.435} & \textbf{0.430} & 0.414 & 0.421 &\underline{0.405} &\underline{0.414} & \textbf{0.403} & \textbf{0.413} \\ 
%     &336 & 1.107 & 0.809 & \underline{0.853}& \underline{0.719} & \textbf{0.485} & \textbf{0.461} & 0.440 & 0.440 & \underline{0.429} & \underline{0.430} & \textbf{0.427} & \textbf{0.428} \\ 
%     &720 & 1.181 & 0.865 & \underline{0.914} & \underline{0.741} & \textbf{0.534} & \textbf{0.524} & 0.460 & 0.473 & \underline{0.435} & \underline{0.455} & \textbf{0.433} & \textbf{0.453} \\ 
%     \hline
       
%       %  \multirow{4}{*}{\rotatebox{90}{ETTm1}} 
%       %  & 96 & 0.672 & 0.571 & \underline{0.435} & \underline{0.444} & \textbf{0.335} & \textbf{0.369} & 0.290 & 0.342 & \underline{0.286} & \underline{0.337} & \textbf{0.283} & \textbf{0.335} \\
%       % & 192 & 0.795 & 0.669 & \underline{0.473} & \underline{0.467} & \textbf{0.380} & \textbf{0.390} & 0.332 & 0.369 & \underline{0.326} & \underline{0.366} & \textbf{0.322} & \textbf{0.363} \\
%       % & 336 & 1.212 & 0.871 & \underline{0.545} & \underline{0.518} & \textbf{0.423} & \textbf{0.426} & 0.366 & 0.392 & \underline{0.359} & \underline{0.388} & \textbf{0.356} & \textbf{0.385} \\
%       % & 720 & 1.166 & 0.823 & \underline{0.669} & \underline{0.589} & \textbf{0.505} & \textbf{0.480} & 0.420 & 0.424 & \underline{0.408} & \textbf{0.413} & \textbf{0.407} & \underline{0.417} \\
%       % \hline
%        \multirow{4}{*}{\rotatebox{90}{Weather}} 
%        &  96 & 0.300 & 0.384 & \underline{0.277} & \underline{0.354} & \textbf{0.179}& \textbf{0.249} & 0.152 & 0.199 & \underline{0.149} & \underline{0.197} & \textbf{0.144} & \textbf{0.194} \\
%         &192 & 0.598 & 0.544 & \underline{0.407} & \underline{0.447} & \textbf{0.226} & \textbf{0.296} & 0.197 & 0.243 & \underline{0.192} & \textbf{0.238} & \textbf{0.189} & \textbf{0.238} \\ 
%         &336 & 0.578 & 0.523 & \underline{0.529} & \underline{0.520}& \textbf{0.276} & \textbf{0.334} & 0.250 & 0.284 & \underline{0.247}& \underline{0.280} & \textbf{0.239} & \textbf{0.279} \\ 
%        &720 & 1.059 & 0.741 & \underline{0.951} & \underline{0.734} & \textbf{0.332} & \textbf{0.372} & \underline{0.320} & 0.335 & 0.321 & \underline{0.332} & \textbf{0.312} & \textbf{0.331} \\  \hline
%       \label{tab:ablation}
% \end{tabular}
% \end{table*}

\subsection{Effect of Hyper-Parameters}

We investigate the impact of the hyper-parameter $\beta$ on the ETTh1 and ETTm2 datasets with two baselines. In Figure~\ref{fig:ablation_beta} (a) (b),
% we increase the value of $\beta$ from $0$ to {$1e^{5}$ and evaluate MSE with different prediction windows on two datasets and two baselines. 
we vary the value of $\beta$ from $0$ to $1e^{5}$ and evaluate the MSE with different prediction windows for both datasets and baselines.
We find that when $\beta$ is small, baselines exhibit poor and unstable performance. As $\beta$ increases, baselines demonstrate improved and more stable performance. Furthermore, as the prediction window increases, the overfitting problem s become more severe for baselines. 
Therefore, a larger $\beta$ is needed to remove superfluous information and mitigate overfitting. 
Additionally, we evaluate $\lambda$ with PatchTST and RMLP. We observe that a larger $\lambda$ leads to better performance for these models. Moreover, when $\lambda \geq 0.8$, the performance stabilizes. 
%the better models' performance, and when $\lambda \geq 0.8$, the performance is stable. 

%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.41]{figure/param_beta_lamb.pdf}
%\caption{Evaluation on hyper-parameter $\beta$ and $\lambda$. We evaluate the impact of $\beta$ with Informer and Stationary on the ETTh1 and ETTm2 datasets, we evaluate $\lambda$ with PatchTST and RMLP on the ETTh1. }
%\label{fig:ablation_beta}
%\end{figure}










==> icml2024/section/intro.tex <==
\section{Introduction}
Multivariate time series forecasting (MTSF) plays a pivotal role in diverse applications ranging from  traffic flow estimation~\citep{bai2020adaptive}, weather prediction~\citep{chen2021autoformer}, energy consumption~\citep{zhou2021informer} and healthcare~\citep{bahadori2019temporal}. Deep learning has ushered in a new era for MTSF, with methodologies rooted in RNN-based~\citep{franceschi2019unsupervised, ijcai18Liu, salinas2020deepar, rangapuram2018deep} and CNN-based models~\citep{lea2017temporal, lai2018modeling}, that surpass the performance metrics set by traditional techniques~\citep{box2015time}. A notable breakthrough has been the advent of Transformer-based models~\citep{li2019enhancing, zhou2021informer, chen2021autoformer, zhou2022fedformer}. Equipped with attention mechanisms, these models adeptly seize long-range temporal dependencies, establishing a new benchmark for forecasting efficacy. While their primary intent is to harness multivariate correlations, recent research indicates a potential shortcoming: these models might not sufficiently discern cross-variable dependencies~\citep{murphy2022univariate,nie2022time,zeng2022transformers}. This has spurred initiatives to tease out single variable information for more nuanced forecasting.



%Transformer-based models  Due to the attention mechanism which has the ability to capture long-range dependencies, Transformer-based models~\citep{li2019enhancing, zhou2021informer, chen2021autoformer, zhou2022fedformer} have been recently proposed to catch long-term temporal correlation in time series forecasting and have shown promising performance. These models aim to capture multivariate correlations. Recently, several studies~\citep{murphy2022univariate,nie2022time,zeng2022transformers} argue that these models fail to adequately learn cross-variable dependencies and have proposed to extract single variable information. 
%Channel-Independent models which outperform Channel-Dependent models. However, the improvement is based on the sacrifice of cross-variable information.  

When it comes to modeling variable dependencies, MTSF models can be broadly classified into two categories: Channel-mixing models and Channel-independence models, as highlighted in  Figure~\ref{fig:intro_example}~(a)~\citep{nie2022time}. Specifically, Channel-mixing models ingest all features from the time series, projecting them into an embedding space to blend information. Conversely, Channel-independence models restrict their input token to information sourced from just one channel.
%Among them, the Channel-Independent models only takes \textcolor{red}{take} the historical series of the corresponding variable as input when predicting the future series of $i$-th variable; while the Channel-Dependent models take the historical series of $m$ variables as input, where $m \leq C$ and $C$ is the number of variables. 
Recent studies~\citep{murphy2022univariate,nie2022time,zeng2022transformers} indicates that Channel-independence models significantly outpace Channel-mixing models on certain datasets. Yet, this advantage comes with a trade-off: the omission of crucial cross-variable information. Such an omission can be detrimental, especially when the variables inherently correlate. Illustratively, Figure~\ref{fig:intro_example}~(b) showcases traffic flow variations from six proximate detectors in the PEMS08 dataset~\citep{chen2001freeway} . A discernible trend emerges across these detectors, suggesting that exploiting their interrelated patterns could bolster predictive accuracy for future traffic flows. In a comparative experiment, we trained both a Channel-independence model (PatchTST) and a Channel-mixing model (Informer) using the PEMS08 dataset. The outcome, as visualized in Figure~\ref{fig:intro_example} (c), unequivocally shows Informer's superior performance over PatchTST, underscoring the importance of cross-variable insights. Motivated by these findings, we introduce the \textbf{C}ross-Variable \textbf{D}ecorrelation \textbf{A}ware Feature \textbf{M}odeling (\mf) for Channel-mixing methodologies. \mf~ aims to hone in on cross-variable information and prune redundant data. It achieves this by minimizing mutual information between the latent depiction of an individual univariate time series and related multivariate inputs, while concurrently amplifying the shared mutual information between the latent model, its univariate input, and the subsequent univariate forecast.




%We also train a Channel-independence model (PatchTST) and a Channel-mixing model (Informer) on the PEMS08 dataset. The experimental results are shown in Figure~\ref{fig:intro_example} (c), we observe that Informer outperforms PatchTST in a large margin which demonstrates the importance of cross-variable information. Therefore, to extract cross-variable information while eliminating superfluous information, we introduce \textbf{C}ross-Variable \textbf{D}ecorrelation \textbf{A}ware Feature \textbf{M}odeling (\mf) for the channel-mixing methods, which minimizes the mutual information between the latent representation of one single univariate time series and other multivariate series input to remove superfluous information while maximizing the joint mutual information among the latent representation, its univariate input and the corresponding univariate predicted series.

Apart from modeling channel dependence, another significant challenge in MTSF is the accumulation of errors along time, as shown in Figure~\ref{fig:intro_example}~(a).  To mitigate this, a number of studies~\citep{nie2022time,zeng2022transformers,zhou2021informer,zhang2023crossformer} have adopted a direct forecasting strategy using a single-step forecaster {that generates multi-step predictions in a single step}, typically configured as a fully-connected network. Although often superior to auto-regressive forecasters, this method tends to neglect the temporal correlations across varied timesteps in the target series, curtailing its potential to capture series inter-dependencies effectively. Drawing inspiration from the notable temporal relationships observed in adjacent sub-sequences post-downsampling~\citep{liu2022scinet}, we propose \textbf{T}emporal Correlation \textbf{A}ware \textbf{M}odeling (\ms), which  iteratively down-samples and optimizes mutual information between consecutive sub-sequences of both the forecasted and target series.


%On the other hand, to alleviate the error accumulation effects, as shown in Figure~\ref{fig:intro_example} (a), previous studies~\citep{nie2022time,zeng2022transformers,zhou2021informer,zhang2023crossformer} directly predict the future series with the single-step forecaster which is usually a fully-connected network. Compared to auto-regressive forecaster, although the single-step forecaster performs better, it ignores the temporal correlations of different timesteps in the target series, thus resulting in insufficient ability to model target series dependencies. Motivated by the observation that adjacent sub-sequences after downsampling have large temporal relationships~\citep{liu2022scinet}, we propose \textbf{T}emporal Correlation \textbf{A}ware \textbf{M}odeling (\ms), which continuously downsamples and maximizes the mutual information between the adjacent sub-sequences of the predicted series and the target series.

%In this paper, We analyze the Channel-Dependent models and Channel-Independent models from the perspective of Mutual Information and explain their shortcomings. Mutual Information (MI) is a fundamental measure of the dependence between two variables. The definition of MI between random variable \textcolor{red}{variables} $X$ and Y is:
% \begin{equation}
%     I(X;Y)=\int p(x,y) log \frac{p(x,y)}{p(x)p(y)}dxdy =E_{p(x,y)} \left [log\frac{p(x,y)}{p(x)p(y)} \right ]
% \end{equation}
% The framework of Channel-Dependent models and Channel-Independent models is shown in Figure~\ref{fig:intro_example} (a). Given the historical time series $X=\{X_{t-T+1}^{c},...,X_{t}^{c}\}_{c=1}^{C}$, where $T$ and $C$ represent the number of historical time steps and variables, respectively. These models generally extract feature $Z=\{ Z^{1},...,Z^{C} \}$, and then use latent representation $Z$ to generate future time series $Y=\{Y_{t+1}^{c},...,Y_{t+P}^{c}\}_{c=1}^{C}$. This paper endeavors to investigate the following aspects and offer appropriate solutions from the perspective of Mutual Information: 
% %The Channel-Dependent models maximize the MI between historical series $X$ and latent representations $Z$ , which can be formulated as $max\,\, I_{\theta}(X;Z^{i})$. On the contrary, Channel-Independent models ignore cross-variable dependencies. Therefore, for the Channel-Independent models, the MI between $X^{j}$ and $Z^{i}$ is $0$, which was formulated as $I_{\theta}(x^{j};Z^{i})_{\{i \neq j\}}= 0$.
%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.42]{figure/intro_example7.pdf}
%\caption{(a) The framework of Channel-independence models and Channel-mixing models. Given historical series $X=\{X^i\}$ where $i$ denotes the channel index, the Channel-mixing model tends to maximize the mutual information between $X$ and the latent representation $Z^{i}$, and the mutual information between $Z^{i}$ and the i-th future series $Y^{i}$. The Channel-independence models maximize the mutual information between the i-th historical series $X^{i}$ and $Z^{i}$  while ignoring the mutual information between $Z^{i}$ and other channels; (b) Traffic flow of 5 adjacent detectors in the PEMS08 dataset; and (c) Prediction results of 
% Channel-independence model (PatchTST), Channel-mixing model(Informer), and that with our framework, respectively.}
%\label{fig:intro_example}
%\end{figure}


\begin{figure*}
\centering
\begin{minipage}{1.3\columnwidth}
    \subfloat[\scriptsize The Framework of Channel-Independence and Channel-mixing models]{
      \label{c} 
      \includegraphics[width=1.00\columnwidth]{figure/frame/fram.pdf}}
\end{minipage}
\begin{minipage}{0.7\columnwidth}
    \subfloat[\scriptsize \centering Traffic flow of 5 adjacent detectors in PEMS08]{
      \label{a} 
      \includegraphics[width=1.0\columnwidth]{figure/frame/pems08.pdf}}\\
    \subfloat[\scriptsize \centering Prediction results of PatchTST and Informer in PEMS08]{
      \label{b} 
      \includegraphics[width=1.0\columnwidth]{figure/frame/pems08_pred.pdf}}
\end{minipage}
\caption{(a) The framework of Channel-independence models and Channel-mixing models. Given historical series $X=\{X^i\}$ where $i$ denotes the channel index, the Channel-mixing model tends to maximize the mutual information between $X$ and the latent representation $Z^{i}$. Additionally, it maximize the mutual information between $Z^{i}$ and the i-th future series $Y^{i}$. The Channel-independence models maximize the mutual information between the i-th historical series $X^{i}$ and $Z^{i}$  while ignoring the mutual information between $Z^{i}$ and other channels; (b) Traffic flow of 5 adjacent detectors in the PEMS08 dataset; and (c) Prediction results of 
 Channel-independence model (PatchTST), Channel-mixing model (Informer), and that with our framework, respectively.}
\label{fig:intro_example}
\end{figure*}





% \begin{itemize}
%     \item The Channel-Dependent models maximize the Mutual Information between historical variables and features, which can be formulated as $max\,\, I_{\theta}(X;Z^{i})$. On the contrary, Channel-Independent models tend to ignore the cross-variable dependencies. In other words, they assume that the Mutual Information between different variables is $0$, which can be formulated as $I_{\theta}(X^{i};Z^{j})_{\{i \neq j\}}= 0$. Although Channel-Independent models perform better than Channel-Dependent models, it potentially affects models' ability to extract spatial features. As shown in Figure~\ref{fig:intro_example} (b) (c), we demonstrate that the SOTA Channel-Independent model (PatchTST) performs worse than the corresponding Channel-Dependent model on PEMS~\cite{chen2001freeway} dataset with complicated spatial-temporal features. Therefore, in order to extract correctly cross-variable feature and alleviate the overfitting problem, we propose a cross-variable extraction method based on Information Bottleneck named \ms. \ms \textcolor{blue}{uses} the Information Bottleneck theory to control the Mutual Information between cross-variable historical series and latent representation to remove irrelevant cross-variable information and thus reduces overfitting.


    
%     %However, as shown in Figure~\ref{fig:intro_example} (b) (c),
%     %Therefore, for the Channel-Independent models, the MI between variables is zero, which was formulated as $I_{\theta}(X^{i};Z^{j})_{\{i \neq j\}}= 0$. 
%     %However, \textcolor{blue}{different channels are not completely unrelated.} As shown in Table~\ref{tab:rho}, we use the Pearson Correlation Coefficient between historical and future series of the same variable and different variables, respectively. We find that there is still a weak to moderate correlation historical and future series of different variables.
    
%     \item To alleviate the error accumulation effects, as shown in Figure~\ref{fig:intro_example} (a), previous works~\cite{nie2022time,zeng2022transformers,zhou2021informer,zhang2023crossformer} use a single-step forecaster which is usually a fully-connected network to predict the future series. Compared to auto-regressive forecaster, although the single-step forecaster performs better, it ignores the relationship between future time steps which means that $I(Y_{j}^{i},Y_{k}^{i})_{\{ j\neq k \}}=0$, thus resulting insufficient ability to model future series dependencies. Motivated by the observation that adjacent sub-sequences after downsampling have large temporal relationships, we propose \mf, which tends to improve the models' ability to capture future temporal relationships by continuously downsampling and maximizing the Mutual Information between adjacent sub-sequences.
%     %As shown in Figure~\ref{}, we divide a series into two parts of equal length in three ways, and we find that the adjacent subsequences generated by downsampling have a strong correlation compared with random sampling and time order sampling. Therefore, we enhance the correlation between future time steps by enhancing the Mutual Information between the downsampling subsequences.
% \end{itemize}

% (1) The Channel-Dependent models maximize the Mutual Information between historical variables and features, which can be formulated as $max\,\, I_{\theta}(X;Z^{i})$. On the contrary, Channel-Independent models tend to ignore the cross-variable dependencies. In other words, they assume that the Mutual Information between different variables is $0$, which can be formulated as $I_{\theta}(X^{i};Z^{j})_{\{i \neq j\}}= 0$. Although Channel-Independent models perform better than Channel-Dependent models, it potentially affects \textcolor{red}{the} models' ability to extract spatial features. As shown in Figure~\ref{fig:intro_example} (b) (c), we demonstrate that the SOTA Channel-Independent model (PatchTST) performs worse than the corresponding Channel-Dependent model on PEMS~\cite{chen2001freeway} dataset with complicated spatial-temporal features. Therefore, in order to extract correctly cross-variable feature \textcolor{red}{features} and alleviate the overfitting problem, we propose a cross-variable extraction method based on Information Bottleneck named \ms. \ms \xspace\textcolor{blue}{uses} the Information Bottleneck theory to control the Mutual Information between cross-variable historical series and latent representation to remove irrelevant cross-variable information and thus reduces overfitting.


    
    %However, as shown in Figure~\ref{fig:intro_example} (b) (c),
    %Therefore, for the Channel-Independent models, the MI between variables is zero, which was formulated as $I_{\theta}(X^{i};Z^{j})_{\{i \neq j\}}= 0$. 
    %However, \textcolor{blue}{different channels are not completely unrelated.} As shown in Table~\ref{tab:rho}, we use the Pearson Correlation Coefficient between historical and future series of the same variable and different variables, respectively. We find that there is still a weak to moderate correlation historical and future series of different variables.
    
% (2) To alleviate the error accumulation effects, as shown in Figure~\ref{fig:intro_example} (a), previous works~\cite{nie2022time,zeng2022transformers,zhou2021informer,zhang2023crossformer} use a single-step forecaster which is usually a fully-connected network to predict the future series. Compared to auto-regressive forecaster, although the single-step forecaster performs better, it ignores the relationship between future time steps which means that $I(Y_{j}^{i},Y_{k}^{i})_{\{ j\neq k \}}=0$, thus resulting  \textcolor{red}{in} insufficient ability to model future series dependencies. Motivated by the observation that adjacent sub-sequences after downsampling have large temporal relationships, we propose \mf, which tends to improve the models' ability to capture future temporal relationships by continuously downsampling and maximizing the Mutual Information between adjacent sub-sequences.
    %As shown in Figure~\ref{}, we divide a series into two parts of equal length in three ways, and we find that the adjacent subsequences generated by downsampling have a strong correlation compared with random sampling and time order sampling. Therefore, we enhance the correlation between future time steps by enhancing the Mutual Information between the downsampling subsequences.


In essence, this paper delves into two pivotal challenges in multivariate time series forecasting: \textbf{cross-variable relationships} and \textbf{temporal relationships}. Drawing inspiration from these challenges, we develop a novel framework, denoted as  \framework \xspace. This framework seamlessly integrates \mf \xspace and \ms. Our paper's key contributions encompass:

%In summary, this paper explores two key challenges in multivariate time series forecasting: \textbf{cross-variable relationships} and \textbf{temporal relationships}. Motivated by the above, we develop a novel framework named \framework \xspace with \mf \xspace and \ms. The main contributions of this paper are as follows:
% \begin{itemize}
%     \item We propose \mf, which can eliminate irrelevant cross-variable information and alleviate the overfitting problem by controlling the Mutual Information between Multivariate historical series and the latent representation.
%     \item To enhance the models' ability to extract temporal relationships of future series, we propose \mf, which learns the temporal relationships by downsampling and maximizing the Mutual Information of adjacent sub-sequences.
%     \item Combining \mf \xspace and \ms, we propose \framework 
% \end{itemize}

\begin{itemize}
    \item We introduce \textbf{C}ross-Variable \textbf{D}ecorrelation \textbf{A}ware Feature \textbf{M}odeling (\mf) designed specifically for Channel-mixing methods. It adeptly distills cross-variable information, simultaneously filtering out superfluous information.
    \item Our proposed \textbf{T}emporal Correlation \textbf{A}ware \textbf{M}odeling (\ms) is tailored to effectively capture the temporal correlations across varied timesteps in the target series.
    \item Synthesizing  \mf \xspace and \ms, we unveil a cutting-edge framework for MTSF, denominated as  \framework.
\end{itemize}

Through rigorous experimentation on diverse real-world datasets, it's evident that our \framework  \xspace consistently eclipses existing Channel-mixing benchmarks, achieving superior accuracy and notably mitigating overfitting. Furthermore, \framework \xspace enhances the efficacy of Channel-Independent models, especially in instances with ambiguous cross-variable traits. 


==> icml2024/section/related_work.tex <==
\section{Related Work}

\subsection{Multivariate Time Series Forecasting}

Multivariate time series forecasting is the task of predicting future values of variables, given historical observations. With the development of deep learning, various neural models have been proposed and demonstrated promising performance in this task. RNN-based~\citep{franceschi2019unsupervised, salinas2020deepar, rangapuram2018deep} and CNN-based~\citep{lea2017temporal, lai2018modeling} models are proposed for models time series data using RNN or CNN respectively, but these models have difficulty in modeling long-term dependency. In recent years, a large body of works try to apply Transformer models to forecast long-term multivariate series and have shown great potential~\citep{li2019enhancing, zhou2021informer, chen2021autoformer, zhou2022fedformer, nie2022time}, Especially, LogTrans~\citep{li2019enhancing} proposes the LogSparse attention in order to reduce the complexity from $O(L^{2})$ to $O(L(\log L)^{2})$. Informer~\citep{zhou2021informer} utilizes the sparsity of attention score through KL-divergence estimation and proposes ProbSparse self-attention mechanism which achieves $O(L\log L)$ complexity. Autoformer~\citep{chen2021autoformer} introduces a decomposition architecture with the Auto-Correlation mechanism to capture the seasonal and trend features of historical series which also achieves $O(L\log L)$ complexity and has a better performance. Afterword, FEDformer~\citep{zhou2022fedformer} employs the mixture-of-expert to enhance the seasonal-trend decomposition and achieves $O(L)$ complexity. The above methods focus on modeling temporal dependency yet omit the correlation of different variables. Crossformer~\citep{zhang2023crossformer} introduces Two-Stage Attention to effectively capture the cross-time and cross-dimension dependency. But the effectiveness of Crossformer is limited. 
%because the previous methods have implicitly captured the cross-dimension dependency. 
Recently, several works~\citep{murphy2022univariate, nie2022time,zeng2022transformers} observe that modeling cross-dimension dependency makes neural models suffer from overfitting in most benchmarks, therefore, they propose Channel-Independence methods to avoid this issue. However, the improvement is based on the sacrifice of cross-variable information. Besides, existing models primarily focus on extracting correlations of historical series while disregarding the correlations of target series.

\subsection{Mutual Information and Information Bottleneck}
Mutual Information (MI) is an entropy-based measure that quantifies the dependence between random variables which has the form:
\begin{equation}
    I(X;Y)=\int p(x,y) log \frac{p(x,y)}{p(x)p(y)}dxdy %=E_{p(x,y)} \left [log\frac{p(x,y)}{p(x)p(y)} \right ]
\end{equation}
Mutual Information was used in a wide range of domains and tasks, including feature selection~\citep{kwak2002input}, causality~\citep{butte1999mutual}, and Information Bottleneck~\citep{tishby2000information}. Information Bottleneck (IB) was first proposed by~\cite{tishby2000information} which is an information theoretic framework for extracting the most relevant information in the relationship of the input with respect to the output, which can be formulated as $max \,\, I(Y;Z)- \beta I(X;Z)$. Several works~\citep{tishby2015deep, shwartz2017opening} try to use the Information Bottleneck framework to analyze the Deep Neural Networks by quantifying Mutual Information between the network layers and deriving an information theoretic limit on DNN efficiency. Variational Information Bottleneck (VIB) was also proposed~\citep{alemi2016deep} to bridge the gap between Information Bottleneck and deep learning. In recent years, many lower-bound estimations~\citep{belghazi2018mutual, oord2018representation} and upper-bound estimations~\citep{poole2019variational, cheng2020club} have been proposed to estimate MI effectively which are useful to estimate VIB. Nowadays, MI and VIB have been widely used in computer vision~\citep{schulz2020restricting, luo2019significance}, natural language processing~\citep{mahabadi2021variational, west2019bottlesum, voita2019bottom}, reinforcement learning~\citep{goyal2019infobot, igl2019generalization}, and representation learning~\citep{federici2020learning, hjelm2018learning}. However, Mutual Information and Information Bottleneck are less researched in long-term multivariate time-series forecasting.
